Geometrostatics: the geometry of static space-times

We present a new geometric approach to the study of static isolated general relativistic systems for which we suggest the name geometrostatics. After describing the setup, we introduce localized formulas for the ADM-mass and ADM/CMC-center of mass of geometrostatic systems. We then explain the pseudo-Newtonian character of these formulas and show that they converge to Newtonian mass and center of mass in the Newtonian limit, respectively, using Ehlers' frame theory. Moreover, we present a novel physical interpretation of the level sets of the canonical lapse function and apply it to prove uniqueness results. Finally, we suggest a notion of force on test particles in geometrostatic space-times.

==> universe.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(8448,6099)(316,-6406)
\thinlines
{\color[rgb]{0,0,0}\put(2071,-826){\line( 5, 6){225}}
}%
{\color[rgb]{0,0,0}\put(2521,-826){\line(-5, 6){225}}
}%
{\color[rgb]{0,0,0}\put(2386,-5236){\line( 5, 6){225}}
}%
{\color[rgb]{0,0,0}\put(2836,-5236){\line(-5, 6){225}}
}%
{\color[rgb]{0,0,0}\put(2296,-4966){\framebox(6435,4410){}}
}%
\thicklines
{\color[rgb]{1,0,0}\put(2611,-4921){\line( 0, 1){4320}}
}%
\thinlines
{\color[rgb]{0,0,0}\put(2611,-4966){\line( 0,-1){495}}
}%
{\color[rgb]{0,0,0}\put(2701,-4921){\framebox(5985,4320){}}
}%
\thicklines
{\color[rgb]{0,0,0}\put(8461,-4741){\line( 6,-5){270}}
\put(8731,-4966){\line(-6,-5){270}}
}%
\put(2521,-5956){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}0:Newtonian}%
}}}}
\put(2971,-6406){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}theories}%
}}}}
\put(5311,-1771){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}GR}%
}}}}
\put(586,-691){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}\$g, h, T,\$}%
}}}}
\put(316,-1231){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}\$Gamma\$}%
}}}}
\put(8731,-5551){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}\$lambda\$}%
}}}}
\end{picture}%

